Effect of Meltdown and Spectre Patches on the Performance of HPC Applications

In this work we examine how the updates addressing Meltdown and Spectre vulnerabilities impact the performance of HPC applications. To study this we use the application kernel module of XDMoD to test the performance before and after the application of the vulnerability patches. We tested the performance difference for multiple application and benchmarks including: NWChem, NAMD, HPCC, IOR, MDTest and IMB. The results show that although some specific functions can have performance decreased by as much as 74%, the majority of individual metrics indicates little to no decrease in performance. The real-world applications show a 2-3% decrease in performance for single node jobs and a 5-11% decrease for parallel multi node jobs.

==> all_metrics_mega_table.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[!t]
\centering
\footnotesize
\caption{Changes in all measured metrics}
\label{table:all-metrics}
\begin{tabular}
{|L{0.1in}|L{0.6in}|R{0.2in}|L{1.0in}|R{0.3in}|R{0.3in}|R{0.4in}|R{0.4in}|R{0.2in}|R{0.4in}|R{0.4in}|R{0.2in}|L{0.6in}|}
\hline
\multirow{2}{*}{\#} & 
\multirow{2}{*}{Application} & 
\multirow{2}{0.2in}{Nodes} & 
\multirow{2}{1.0in}{Metric} & 
\multirow{2}{0.3in}{Diff., \%} & 
\multirow{2}{0.3in}{Distr. Can be Distin- gui- shed?} & 
\multicolumn{3}{l|}{Before Patch Application} & 
\multicolumn{3}{l|}{After Patch Application} &
\multirow{2}{*}{Units} \\[0.1in]  \cline{7-12} 
 &  &  &  &  &  & 
{\centering Mean, Seconds} &l {\centering Standard Deviation, Seconds} & {Nruns} & 
{\centering Mean, Seconds} & {\centering Standard Deviation, Seconds} & {Nruns} & \\[0.1in] \hline
 
1 & NAMD & 1 & Memory & 0.1 & N & 3.14E+02 & 5.44E-01 & 24 & 3.14E+02 & 6.02E-01 & 56 & MByte \\ \hline
2 & NAMD & 1 & Molecular Dynamics Simulation Performance & -3.5 & Y & 7.67E-10 & 7.11E-12 & 24 & 7.40E-10 & 1.43E-11 & 56 & Second per Day \\ \hline
3 & NAMD & 1 & Wall Clock Time & 3.4 & Y & 3.07E+02 & 1.44E+00 & 24 & 3.17E+02 & 3.05E+00 & 56 & Second \\ \hline
4 & NAMD & 2 & Memory & 0 & N & 3.01E+02 & 3.83E-01 & 22 & 3.01E+02 & 5.08E-01 & 56 & MByte \\ \hline
5 & NAMD & 2 & Molecular Dynamics Simulation Performance & -6.6 & Y & 1.48E-09 & 5.60E-11 & 22 & 1.38E-09 & 8.44E-11 & 56 & Second per Day \\ \hline
6 & NAMD & 2 & Wall Clock Time & 7.2 & Y & 1.75E+02 & 2.78E+00 & 22 & 1.88E+02 & 3.49E+00 & 56 & Second \\ \hline
7 & NWChem & 1 & Global Arrays 'Accumulate' Amount & -0.8 & Y & 1.49E+03 & 1.38E+01 & 23 & 1.47E+03 & 2.14E+01 & 59 & MByte \\ \hline
8 & NWChem & 1 & Global Arrays 'Accumulate' Calls & -1.8 & Y & 7.07E+05 & 1.62E+04 & 23 & 6.94E+05 & 2.06E+04 & 59 & Number of Calls \\ \hline
9 & NWChem & 1 & Global Arrays 'Create' Calls & 0 & N & 5.30E+02 & 3.44E-01 & 23 & 5.30E+02 & 3.78E-01 & 59 & Number of Calls \\ \hline
10 & NWChem & 1 & Global Arrays 'Destroy' Calls & 0 & N & 5.30E+02 & 3.44E-01 & 23 & 5.30E+02 & 3.78E-01 & 59 & Number of Calls \\ \hline
11 & NWChem & 1 & Global Arrays 'Get' Amount & 0 & N & 6.98E+03 & 1.11E+01 & 23 & 6.97E+03 & 1.34E+01 & 59 & MByte \\ \hline
12 & NWChem & 1 & Global Arrays 'Get' Calls & 0 & N & 6.28E+05 & 0.00E+00 & 23 & 6.28E+05 & 2.54E+02 & 59 & Number of Calls \\ \hline
13 & NWChem & 1 & Global Arrays 'Put' Amount & 0 & N & 4.16E+02 & 7.72E-01 & 23 & 4.16E+02 & 9.25E-01 & 59 & MByte \\ \hline
14 & NWChem & 1 & Global Arrays 'Put' Calls & 0 & N & 6.36E+04 & 5.96E+01 & 23 & 6.36E+04 & 8.68E+01 & 59 & Number of Calls \\ \hline
15 & NWChem & 1 & User Time & 1.1 & Y & 7.35E+01 & 7.36E-01 & 23 & 7.43E+01 & 1.08E+00 & 59 & Second \\ \hline
16 & NWChem & 1 & Wall Clock Time & 2.7 & Y & 7.78E+01 & 1.91E+00 & 23 & 7.99E+01 & 1.11E+00 & 59 & Second \\ \hline
17 & NWChem & 2 & Global Arrays 'Accumulate' Amount & -2.6 & Y & 6.91E+02 & 1.61E+01 & 21 & 6.74E+02 & 1.48E+01 & 56 & MByte \\ \hline
18 & NWChem & 2 & Global Arrays 'Accumulate' Calls & -8.6 & Y & 2.25E+05 & 1.65E+04 & 21 & 2.06E+05 & 1.53E+04 & 56 & Number of Calls \\ \hline
19 & NWChem & 2 & Global Arrays 'Create' Calls & 0 & N & 5.30E+02 & 2.18E-01 & 21 & 5.30E+02 & 3.12E-01 & 56 & Number of Calls \\ \hline
20 & NWChem & 2 & Global Arrays 'Destroy' Calls & 0 & N & 5.30E+02 & 2.18E-01 & 21 & 5.30E+02 & 3.12E-01 & 56 & Number of Calls \\ \hline
21 & NWChem & 2 & Global Arrays 'Get' Amount & -0.2 & Y & 3.66E+03 & 9.76E+00 & 21 & 3.66E+03 & 1.19E+01 & 56 & MByte \\ \hline
22 & NWChem & 2 & Global Arrays 'Get' Calls & -0.1 & N & 3.19E+05 & 3.59E+02 & 21 & 3.19E+05 & 4.71E+02 & 56 & Number of Calls \\ \hline
23 & NWChem & 2 & Global Arrays 'Put' Amount & 0 & N & 2.23E+02 & 4.61E-01 & 21 & 2.22E+02 & 4.63E-01 & 56 & MByte \\ \hline
24 & NWChem & 2 & Global Arrays 'Put' Calls & 0 & N & 3.28E+04 & 3.01E+01 & 21 & 3.28E+04 & 3.22E+01 & 56 & Number of Calls \\ \hline
25 & NWChem & 2 & User Time & 10.2 & Y & 4.75E+01 & 8.37E-01 & 21 & 5.23E+01 & 3.84E+00 & 56 & Second \\ \hline
26 & NWChem & 2 & Wall Clock Time & 11.3 & Y & 5.84E+01 & 1.05E+00 & 21 & 6.50E+01 & 4.16E+00 & 56 & Second \\ \hline
27 & HPCC & 1 & Average Double-Precision General Matrix Multiplication (DGEMM) Floating-Point Performance & -1.2 & Y & 8.50E+03 & 5.66E+01 & 23 & 8.40E+03 & 1.11E+02 & 56 & MFLOP per Second \\ \hline
28 & HPCC & 1 & Average STREAM 'Add' Memory Bandwidth & 5 & N & 3.17E+03 & 4.51E+02 & 23 & 3.33E+03 & 5.38E+02 & 56 & MByte per Second \\ \hline
29 & HPCC & 1 & Average STREAM 'Copy' Memory Bandwidth & 3.4 & N & 4.36E+03 & 4.96E+02 & 23 & 4.51E+03 & 5.61E+02 & 56 & MByte per Second \\ \hline
30 & HPCC & 1 & Average STREAM 'Scale' Memory Bandwidth & 3.5 & N & 2.95E+03 & 4.05E+02 & 23 & 3.05E+03 & 4.54E+02 & 56 & MByte per Second \\ \hline
31 & HPCC & 1 & Average STREAM 'Triad' Memory Bandwidth & 8.8 & Y & 3.29E+03 & 5.01E+02 & 23 & 3.58E+03 & 6.68E+02 & 56 & MByte per Second \\ \hline
32 & HPCC & 1 & Fast Fourier Transform (FFTW) Floating-Point Performance & -5.9 & Y & 7.93E+03 & 5.55E+02 & 23 & 7.46E+03 & 1.50E+03 & 56 & MFLOP per Second \\ \hline
33 & HPCC & 1 & High Performance LINPACK Efficiency & -5.4 & Y & 9.26E+01 & 7.86E+00 & 23 & 8.76E+01 & 6.19E+00 & 56 & Percent \\ \hline
34 & HPCC & 1 & High Performance LINPACK Floating-Point Performance & -4.1 & Y & 6.18E+04 & 1.24E+03 & 23 & 5.93E+04 & 1.24E+03 & 56 & MFLOP per Second \\ \hline
35 & HPCC & 1 & High Performance LINPACK Run Time & 4.3 & Y & 8.63E+01 & 1.88E+00 & 23 & 9.00E+01 & 1.97E+00 & 56 & Second \\ \hline
36 & HPCC & 1 & MPI Random Access & -23.3 & Y & 2.09E+00 & 8.59E-02 & 23 & 1.61E+00 & 3.78E-02 & 56 & MUpdate per Second \\ \hline
37 & HPCC & 1 & Parallel Matrix Transpose (PTRANS) & -12.3 & Y & 3.03E+03 & 4.37E+02 & 23 & 2.66E+03 & 8.46E+02 & 56 & MByte per Second \\ \hline
38 & HPCC & 1 & Wall Clock Time & 2.2 & Y & 3.04E+02 & 6.39E+00 & 23 & 3.11E+02 & 4.88E+00 & 56 & Second \\ \hline
39 & HPCC & 2 & Average Double-Precision General Matrix Multiplication (DGEMM) Floating-Point Performance & -2 & Y & 8.53E+03 & 4.22E+01 & 22 & 8.36E+03 & 9.18E+01 & 56 & MFLOP per Second \\ \hline
40 & HPCC & 2 & Average STREAM 'Add' Memory Bandwidth & 14.1 & Y & 3.12E+03 & 2.91E+02 & 22 & 3.56E+03 & 6.40E+02 & 56 & MByte per Second \\ \hline
41 & HPCC & 2 & Average STREAM 'Copy' Memory Bandwidth & 10.9 & Y & 4.35E+03 & 3.16E+02 & 22 & 4.82E+03 & 6.27E+02 & 56 & MByte per Second \\ \hline
42 & HPCC & 2 & Average STREAM 'Scale' Memory Bandwidth & 13.8 & Y & 2.92E+03 & 3.09E+02 & 22 & 3.32E+03 & 5.95E+02 & 56 & MByte per Second \\ \hline
43 & HPCC & 2 & Average STREAM 'Triad' Memory Bandwidth & 16.5 & Y & 3.21E+03 & 3.28E+02 & 22 & 3.75E+03 & 6.94E+02 & 56 & MByte per Second \\ \hline
44 & HPCC & 2 & Fast Fourier Transform (FFTW) Floating-Point Performance & -6.4 & Y & 1.23E+04 & 6.35E+02 & 22 & 1.16E+04 & 1.65E+03 & 56 & MFLOP per Second \\ \hline
45 & HPCC & 2 & High Performance LINPACK Efficiency & -12.4 & Y & 9.62E+01 & 1.01E+01 & 22 & 8.42E+01 & 7.16E+00 & 56 & Percent \\ \hline
46 & HPCC & 2 & High Performance LINPACK Floating-Point Performance & -8.6 & Y & 1.22E+05 & 4.85E+02 & 22 & 1.11E+05 & 2.75E+03 & 56 & MFLOP per Second \\ \hline
47 & HPCC & 2 & High Performance LINPACK Run Time & 9.5 & Y & 1.24E+02 & 4.94E-01 & 22 & 1.35E+02 & 3.42E+00 & 56 & Second \\ \hline
48 & HPCC & 2 & MPI Random Access & -54 & Y & 9.59E+00 & 3.29E-01 & 22 & 4.41E+00 & 2.69E-01 & 56 & MUpdate per Second \\ \hline
49 & HPCC & 2 & Parallel Matrix Transpose (PTRANS) & -9.6 & Y & 2.62E+03 & 1.87E+02 & 22 & 2.36E+03 & 3.44E+02 & 56 & MByte per Second \\ \hline
50 & HPCC & 2 & Wall Clock Time & 5.5 & Y & 3.45E+02 & 5.41E+00 & 22 & 3.64E+02 & 8.44E+00 & 56 & Second \\ \hline
51 & IMB & 2 & Max Exchange Bandwidth & 0.2 & N & 3.90E+03 & 3.60E+01 & 21 & 3.91E+03 & 6.30E+01 & 56 & MByte per Second \\ \hline
52 & IMB & 2 & Max MPI-2 Bidirectional 'Get' Bandwidth (aggregate) & -0.7 & N & 1.99E+03 & 4.31E+01 & 21 & 1.98E+03 & 5.40E+01 & 56 & MByte per Second \\ \hline
53 & IMB & 2 & Max MPI-2 Bidirectional 'Get' Bandwidth (non-aggregate) & -2.8 & Y & 2.11E+03 & 5.71E+01 & 21 & 2.05E+03 & 4.68E+01 & 56 & MByte per Second \\ \hline
54 & IMB & 2 & Max MPI-2 Bidirectional 'Put' Bandwidth (aggregate) & 0.4 & N & 2.05E+03 & 6.51E+01 & 21 & 2.06E+03 & 3.02E+01 & 56 & MByte per Second \\ \hline
55 & IMB & 2 & Max MPI-2 Bidirectional 'Put' Bandwidth (non-aggregate) & -1.7 & Y & 2.12E+03 & 3.61E+01 & 21 & 2.08E+03 & 4.37E+01 & 56 & MByte per Second \\ \hline
56 & IMB & 2 & Max MPI-2 Unidirectional 'Get' Bandwidth (aggregate) & -0.1 & N & 3.10E+03 & 1.45E+01 & 21 & 3.10E+03 & 8.30E+00 & 56 & MByte per Second \\ \hline
57 & IMB & 2 & Max MPI-2 Unidirectional 'Get' Bandwidth (non-aggregate) & -1 & Y & 2.93E+03 & 5.45E+01 & 21 & 2.90E+03 & 5.59E+01 & 56 & MByte per Second \\ \hline
58 & IMB & 2 & Max MPI-2 Unidirectional 'Put' Bandwidth (aggregate) & 0 & N & 3.12E+03 & 6.18E+00 & 21 & 3.12E+03 & 7.70E+00 & 56 & MByte per Second \\ \hline
59 & IMB & 2 & Max MPI-2 Unidirectional 'Put' Bandwidth (non-aggregate) & -1.1 & Y & 2.96E+03 & 4.11E+01 & 21 & 2.92E+03 & 5.11E+01 & 56 & MByte per Second \\ \hline
60 & IMB & 2 & Max PingPing Bandwidth & -0.1 & N & 2.60E+03 & 3.43E+01 & 21 & 2.60E+03 & 3.00E+01 & 56 & MByte per Second \\ \hline
61 & IMB & 2 & Max PingPong Bandwidth & -0.1 & N & 3.08E+03 & 9.99E+00 & 21 & 3.08E+03 & 7.15E+00 & 56 & MByte per Second \\ \hline
62 & IMB & 2 & Max SendRecv Bandwidth & -0.4 & N & 5.22E+03 & 7.35E+01 & 21 & 5.20E+03 & 7.24E+01 & 56 & MByte per Second \\ \hline
63 & IMB & 2 & Min AllGather Latency & 1.5 & Y & 2.54E-06 & 5.12E-08 & 21 & 2.58E-06 & 6.88E-08 & 56 & Second \\ \hline
64 & IMB & 2 & Min AllGatherV Latency & -1 & N & 2.99E-06 & 1.16E-07 & 21 & 2.96E-06 & 6.92E-08 & 56 & Second \\ \hline
65 & IMB & 2 & Min AllReduce Latency & -2.3 & Y & 3.02E-06 & 1.22E-07 & 21 & 2.95E-06 & 7.10E-08 & 56 & Second \\ \hline
66 & IMB & 2 & Min AllToAll Latency & 0.9 & Y & 2.53E-06 & 3.66E-08 & 21 & 2.55E-06 & 3.56E-08 & 56 & Second \\ \hline
67 & IMB & 2 & Min AllToAllV Latency & 3.8 & Y & 3.21E-06 & 3.01E-08 & 21 & 3.33E-06 & 1.14E-07 & 56 & Second \\ \hline
68 & IMB & 2 & Min Barrier Latency & 3.3 & Y & 2.41E-06 & 8.48E-08 & 21 & 2.48E-06 & 1.24E-07 & 56 & Second \\ \hline
69 & IMB & 2 & Min Broadcast Latency & -0.7 & N & 2.40E-06 & 2.53E-08 & 21 & 2.39E-06 & 8.71E-08 & 56 & Second \\ \hline
70 & IMB & 2 & Min Gather Latency & -0.4 & N & 2.60E-06 & 9.05E-08 & 21 & 2.59E-06 & 3.39E-08 & 56 & Second \\ \hline
71 & IMB & 2 & Min GatherV Latency & 0.9 & N & 2.44E-06 & 2.10E-08 & 21 & 2.46E-06 & 8.03E-08 & 56 & Second \\ \hline
72 & IMB & 2 & Min MPI-2 'Accumulate' Latency (aggregate) & 0.5 & N & 1.00E-06 & 7.08E-08 & 21 & 1.01E-06 & 6.05E-08 & 56 & Second \\ \hline
73 & IMB & 2 & Min MPI-2 'Accumulate' Latency (non-aggregate) & 1.8 & N & 6.29E-06 & 2.50E-07 & 21 & 6.40E-06 & 3.00E-07 & 56 & Second \\ \hline
74 & IMB & 2 & Min MPI-2 Window Creation Latency & 0.3 & N & 2.44E-05 & 1.36E-07 & 21 & 2.45E-05 & 2.06E-07 & 56 & Second \\ \hline
75 & IMB & 2 & Min Reduce Latency & 3.5 & Y & 2.74E-06 & 6.69E-08 & 21 & 2.84E-06 & 1.05E-07 & 56 & Second \\ \hline
76 & IMB & 2 & Min ReduceScatter Latency & 0.8 & N & 1.65E-06 & 8.98E-08 & 21 & 1.67E-06 & 1.03E-07 & 56 & Second \\ \hline
77 & IMB & 2 & Min Scatter Latency & 1.6 & Y & 2.58E-06 & 1.60E-08 & 21 & 2.63E-06 & 5.97E-08 & 56 & Second \\ \hline
78 & IMB & 2 & Min ScatterV Latency & 0.1 & N & 2.54E-06 & 7.85E-08 & 21 & 2.54E-06 & 4.09E-08 & 56 & Second \\ \hline
79 & IMB & 2 & Wall Clock Time & 4 & Y & 1.48E+01 & 5.39E-01 & 21 & 1.54E+01 & 1.39E+00 & 56 & Second \\ \hline
80 & IOR & 1 & HDF5 Collective N-to-1  File Close Time (Read) & 23.2 & N & 1.59E-01 & 5.45E-02 & 21 & 1.95E-01 & 1.07E-01 & 55 & Second \\ \hline
81 & IOR & 1 & HDF5 Collective N-to-1  File Close Time (Write) & -18.3 & N & 6.04E-01 & 3.70E-01 & 21 & 4.93E-01 & 1.88E-01 & 55 & Second \\ \hline
82 & IOR & 1 & HDF5 Collective N-to-1  File Open Time (Read) & -21.3 & N & 2.46E-01 & 2.16E-01 & 21 & 1.93E-01 & 4.08E-02 & 55 & Second \\ \hline
83 & IOR & 1 & HDF5 Collective N-to-1  File Open Time (Write) & 45.7 & N & 7.57E-02 & 2.94E-03 & 21 & 1.10E-01 & 1.42E-01 & 55 & Second \\ \hline
84 & IOR & 1 & HDF5 Collective N-to-1 Read Aggregate Throughput & -0.4 & N & 2.60E+02 & 1.37E+01 & 21 & 2.59E+02 & 2.13E+01 & 55 & MByte per Second \\ \hline
85 & IOR & 1 & HDF5 Collective N-to-1 Write Aggregate Throughput & -4.1 & N & 1.13E+02 & 1.21E+01 & 21 & 1.08E+02 & 7.75E+00 & 55 & MByte per Second \\ \hline
86 & IOR & 1 & HDF5 Independent N-to-1  File Close Time (Read) & 15.3 & N & 6.32E+00 & 2.24E+00 & 21 & 7.28E+00 & 2.11E+00 & 55 & Second \\ \hline
87 & IOR & 1 & HDF5 Independent N-to-1  File Close Time (Write) & 5.1 & N & 4.39E+00 & 9.46E-01 & 21 & 4.62E+00 & 1.00E+00 & 55 & Second \\ \hline
88 & IOR & 1 & HDF5 Independent N-to-1  File Open Time (Read) & 36.9 & N & 2.13E-01 & 1.30E-01 & 21 & 2.92E-01 & 2.88E-01 & 55 & Second \\ \hline
89 & IOR & 1 & HDF5 Independent N-to-1  File Open Time (Write) & 0.5 & N & 1.65E-01 & 2.06E-01 & 21 & 1.66E-01 & 2.12E-01 & 55 & Second \\ \hline
90 & IOR & 1 & HDF5 Independent N-to-1 Read Aggregate Throughput & -6.3 & N & 1.64E+02 & 2.17E+01 & 21 & 1.53E+02 & 2.04E+01 & 55 & MByte per Second \\ \hline
91 & IOR & 1 & HDF5 Independent N-to-1 Write Aggregate Throughput & -3.7 & N & 1.66E+02 & 2.67E+01 & 21 & 1.60E+02 & 2.26E+01 & 55 & MByte per Second \\ \hline
92 & IOR & 1 & HDF5 N-to-N  File Close Time (Read) & -5.3 & N & 6.20E+00 & 8.35E-01 & 21 & 5.87E+00 & 8.94E-01 & 55 & Second \\ \hline
93 & IOR & 1 & HDF5 N-to-N  File Close Time (Write) & 6.8 & N & 5.94E+00 & 1.52E+00 & 21 & 6.34E+00 & 1.83E+00 & 54 & Second \\ \hline
94 & IOR & 1 & HDF5 N-to-N  File Open Time (Read) & -12.7 & N & 2.28E+00 & 6.08E-01 & 21 & 1.99E+00 & 9.10E-01 & 55 & Second \\ \hline
95 & IOR & 1 & HDF5 N-to-N  File Open Time (Write) & -1.9 & N & 4.70E+00 & 1.86E+00 & 21 & 4.61E+00 & 1.61E+00 & 54 & Second \\ \hline
96 & IOR & 1 & HDF5 N-to-N Read Aggregate Throughput & 2.9 & N & 2.14E+02 & 1.60E+01 & 21 & 2.20E+02 & 1.80E+01 & 55 & MByte per Second \\ \hline
97 & IOR & 1 & HDF5 N-to-N Write Aggregate Throughput & 0.5 & N & 2.20E+02 & 2.12E+01 & 21 & 2.21E+02 & 2.73E+01 & 54 & MByte per Second \\ \hline
98 & IOR & 1 & MPIIO Collective N-to-1  File Close Time (Read) & -11.4 & N & 2.23E-01 & 6.46E-02 & 21 & 1.98E-01 & 6.16E-02 & 55 & Second \\ \hline
99 & IOR & 1 & MPIIO Collective N-to-1  File Close Time (Write) & 22.7 & N & 6.54E-01 & 2.78E-01 & 21 & 8.03E-01 & 6.21E-01 & 55 & Second \\ \hline
100 & IOR & 1 & MPIIO Collective N-to-1  File Open Time (Read) & 1.6 & Y & 5.72E-02 & 1.63E-03 & 21 & 5.82E-02 & 1.69E-03 & 55 & Second \\ \hline
101 & IOR & 1 & MPIIO Collective N-to-1  File Open Time (Write) & 96.5 & Y & 7.09E-02 & 3.27E-03 & 21 & 1.39E-01 & 1.71E-01 & 55 & Second \\ \hline
102 & IOR & 1 & MPIIO Collective N-to-1 Read Aggregate Throughput & -2.3 & N & 2.70E+02 & 8.86E+00 & 21 & 2.64E+02 & 2.91E+01 & 55 & MByte per Second \\ \hline
103 & IOR & 1 & MPIIO Collective N-to-1 Write Aggregate Throughput & -7.8 & N & 2.31E+02 & 3.89E+01 & 21 & 2.13E+02 & 4.02E+01 & 55 & MByte per Second \\ \hline
104 & IOR & 1 & MPIIO Independent N-to-1  File Close Time (Read) & -1.6 & N & 7.95E+00 & 1.24E+00 & 21 & 7.82E+00 & 1.16E+00 & 55 & Second \\ \hline
105 & IOR & 1 & MPIIO Independent N-to-1  File Close Time (Write) & 9.1 & N & 2.96E+00 & 1.19E+00 & 21 & 3.23E+00 & 1.39E+00 & 55 & Second \\ \hline
106 & IOR & 1 & MPIIO Independent N-to-1  File Open Time (Read) & 2 & Y & 5.59E-02 & 1.81E-03 & 21 & 5.71E-02 & 1.99E-03 & 55 & Second \\ \hline
107 & IOR & 1 & MPIIO Independent N-to-1  File Open Time (Write) & -34.7 & N & 1.62E-01 & 2.42E-01 & 21 & 1.06E-01 & 1.18E-01 & 55 & Second \\ \hline
108 & IOR & 1 & MPIIO Independent N-to-1 Read Aggregate Throughput & -0.5 & N & 1.55E+02 & 1.73E+01 & 21 & 1.54E+02 & 1.49E+01 & 55 & MByte per Second \\ \hline
109 & IOR & 1 & MPIIO Independent N-to-1 Write Aggregate Throughput & -1 & N & 1.89E+02 & 3.77E+01 & 21 & 1.88E+02 & 4.12E+01 & 55 & MByte per Second \\ \hline
110 & IOR & 1 & MPIIO N-to-N  File Close Time (Read) & -9.6 & N & 4.09E+00 & 1.01E+00 & 21 & 3.70E+00 & 9.27E-01 & 55 & Second \\ \hline
111 & IOR & 1 & MPIIO N-to-N  File Close Time (Write) & 33.6 & Y & 4.70E+00 & 2.18E+00 & 21 & 6.28E+00 & 1.90E+00 & 55 & Second \\ \hline
112 & IOR & 1 & MPIIO N-to-N  File Open Time (Read) & 5 & N & 4.24E-01 & 7.89E-01 & 21 & 4.45E-01 & 9.66E-01 & 55 & Second \\ \hline
113 & IOR & 1 & MPIIO N-to-N  File Open Time (Write) & 11.9 & N & 4.05E+00 & 2.48E+00 & 21 & 4.53E+00 & 1.93E+00 & 55 & Second \\ \hline
114 & IOR & 1 & MPIIO N-to-N Read Aggregate Throughput & 1.2 & N & 2.17E+02 & 9.06E+00 & 21 & 2.19E+02 & 1.05E+01 & 55 & MByte per Second \\ \hline
115 & IOR & 1 & MPIIO N-to-N Write Aggregate Throughput & -7.6 & N & 2.62E+02 & 4.77E+01 & 21 & 2.42E+02 & 4.46E+01 & 55 & MByte per Second \\ \hline
116 & IOR & 1 & Number of Tests Passed & -0.2 & N & 1.00E+01 & 0.00E+00 & 21 & 9.98E+00 & 1.35E-01 & 55 & NA \\ \hline
117 & IOR & 1 & Number of Tests Started & -0.1 & N & 2.00E+01 & 0.00E+00 & 21 & 2.00E+01 & 1.35E-01 & 55 & NA \\ \hline
118 & IOR & 1 & Parallel NetCDF Collective N-to-1  File Close Time (Read) & 7.9 & N & 2.98E-01 & 2.19E-01 & 21 & 3.22E-01 & 2.41E-01 & 55 & Second \\ \hline
119 & IOR & 1 & Parallel NetCDF Collective N-to-1  File Close Time (Write) & 2.9 & N & 2.44E-01 & 1.90E-01 & 21 & 2.51E-01 & 1.83E-01 & 55 & Second \\ \hline
120 & IOR & 1 & Parallel NetCDF Collective N-to-1  File Open Time (Read) & 29.5 & N & 5.89E-02 & 1.69E-03 & 21 & 7.64E-02 & 1.19E-01 & 55 & Second \\ \hline
121 & IOR & 1 & Parallel NetCDF Collective N-to-1  File Open Time (Write) & 42.1 & Y & 7.29E-02 & 3.00E-03 & 21 & 1.04E-01 & 1.06E-01 & 55 & Second \\ \hline
122 & IOR & 1 & Parallel NetCDF Collective N-to-1 Read Aggregate Throughput & -0.2 & N & 2.36E+02 & 1.19E+01 & 21 & 2.36E+02 & 1.27E+01 & 55 & MByte per Second \\ \hline
123 & IOR & 1 & Parallel NetCDF Collective N-to-1 Write Aggregate Throughput & -1 & N & 1.98E+02 & 1.47E+01 & 21 & 1.96E+02 & 1.94E+01 & 55 & MByte per Second \\ \hline
124 & IOR & 1 & Parallel NetCDF Independent N-to-1  File Close Time (Read) & -2.3 & N & 2.37E+00 & 8.98E-01 & 21 & 2.32E+00 & 9.69E-01 & 54 & Second \\ \hline
125 & IOR & 1 & Parallel NetCDF Independent N-to-1  File Close Time (Write) & 9.7 & N & 5.78E+00 & 1.59E+00 & 21 & 6.34E+00 & 1.88E+00 & 55 & Second \\ \hline
126 & IOR & 1 & Parallel NetCDF Independent N-to-1  File Open Time (Read) & -7.1 & N & 7.08E-02 & 2.64E-02 & 21 & 6.58E-02 & 1.79E-02 & 54 & Second \\ \hline
127 & IOR & 1 & Parallel NetCDF Independent N-to-1  File Open Time (Write) & 95 & Y & 7.24E-02 & 4.53E-03 & 21 & 1.41E-01 & 2.30E-01 & 55 & Second \\ \hline
128 & IOR & 1 & Parallel NetCDF Independent N-to-1 Read Aggregate Throughput & -1 & N & 2.27E+02 & 6.42E+00 & 21 & 2.25E+02 & 9.63E+00 & 54 & MByte per Second \\ \hline
129 & IOR & 1 & Parallel NetCDF Independent N-to-1 Write Aggregate Throughput & 0.1 & N & 1.56E+02 & 1.78E+01 & 21 & 1.56E+02 & 1.65E+01 & 55 & MByte per Second \\ \hline
130 & IOR & 1 & POSIX N-to-1  File Close Time (Read) & -6.9 & Y & 6.75E+00 & 8.22E-01 & 21 & 6.28E+00 & 1.03E+00 & 55 & Second \\ \hline
131 & IOR & 1 & POSIX N-to-1  File Close Time (Write) & 11.9 & N & 1.03E+00 & 8.06E-01 & 21 & 1.15E+00 & 1.13E+00 & 55 & Second \\ \hline
132 & IOR & 1 & POSIX N-to-1  File Open Time (Read) & -0.1 & N & 2.28E-02 & 1.86E-03 & 21 & 2.28E-02 & 1.69E-03 & 55 & Second \\ \hline
133 & IOR & 1 & POSIX N-to-1  File Open Time (Write) & 35.4 & N & 1.87E-01 & 7.06E-01 & 21 & 2.54E-01 & 9.43E-01 & 55 & Second \\ \hline
134 & IOR & 1 & POSIX N-to-1 Read Aggregate Throughput & 3.3 & N & 1.70E+02 & 1.04E+01 & 21 & 1.75E+02 & 1.41E+01 & 55 & MByte per Second \\ \hline
135 & IOR & 1 & POSIX N-to-1 Write Aggregate Throughput & -0.1 & N & 2.62E+02 & 2.81E+01 & 21 & 2.62E+02 & 3.72E+01 & 55 & MByte per Second \\ \hline
136 & IOR & 1 & POSIX N-to-N  File Close Time (Read) & -3.6 & N & 1.92E+00 & 1.05E+00 & 21 & 1.85E+00 & 1.22E+00 & 55 & Second \\ \hline
137 & IOR & 1 & POSIX N-to-N  File Close Time (Write) & -22.6 & N & 4.60E+00 & 2.14E+00 & 21 & 3.56E+00 & 1.82E+00 & 55 & Second \\ \hline
138 & IOR & 1 & POSIX N-to-N  File Open Time (Read) & 1.2 & N & 1.44E+00 & 1.77E+00 & 21 & 1.45E+00 & 1.75E+00 & 55 & Second \\ \hline
139 & IOR & 1 & POSIX N-to-N  File Open Time (Write) & -28.9 & Y & 4.41E+00 & 2.25E+00 & 21 & 3.14E+00 & 1.99E+00 & 55 & Second \\ \hline
140 & IOR & 1 & POSIX N-to-N Read Aggregate Throughput & 0 & N & 2.32E+02 & 5.47E+00 & 21 & 2.32E+02 & 6.43E+00 & 55 & MByte per Second \\ \hline
141 & IOR & 1 & POSIX N-to-N Write Aggregate Throughput & 14.6 & Y & 2.33E+02 & 4.37E+01 & 21 & 2.67E+02 & 3.47E+01 & 55 & MByte per Second \\ \hline
142 & IOR & 1 & Wall Clock Time & 3.9 & Y & 1.88E+02 & 9.41E+00 & 21 & 1.96E+02 & 1.17E+01 & 55 & Second \\ \hline
143 & IOR & 2 & HDF5 Collective N-to-1  File Close Time (Read) & -29.9 & N & 2.01E-02 & 1.87E-02 & 22 & 1.41E-02 & 3.65E-03 & 56 & Second \\ \hline
144 & IOR & 2 & HDF5 Collective N-to-1  File Close Time (Write) & -9.8 & N & 8.45E-01 & 3.84E-01 & 22 & 7.62E-01 & 3.92E-01 & 56 & Second \\ \hline
145 & IOR & 2 & HDF5 Collective N-to-1  File Open Time (Read) & 20.6 & N & 2.17E-01 & 1.24E-01 & 22 & 2.61E-01 & 1.18E-01 & 56 & Second \\ \hline
146 & IOR & 2 & HDF5 Collective N-to-1  File Open Time (Write) & 3.2 & N & 2.12E-01 & 1.61E-01 & 22 & 2.19E-01 & 1.56E-01 & 56 & Second \\ \hline
147 & IOR & 2 & HDF5 Collective N-to-1 Read Aggregate Throughput & 0.2 & N & 1.87E+02 & 7.19E+00 & 22 & 1.87E+02 & 1.41E+01 & 56 & MByte per Second \\ \hline
148 & IOR & 2 & HDF5 Collective N-to-1 Write Aggregate Throughput & -7.1 & Y & 1.18E+02 & 1.37E+01 & 22 & 1.10E+02 & 9.44E+00 & 56 & MByte per Second \\ \hline
149 & IOR & 2 & HDF5 Independent N-to-1  File Close Time (Read) & 3.3 & N & 9.16E+00 & 2.50E+00 & 22 & 9.47E+00 & 2.02E+00 & 56 & Second \\ \hline
150 & IOR & 2 & HDF5 Independent N-to-1  File Close Time (Write) & 12.2 & N & 8.24E+00 & 2.22E+00 & 22 & 9.25E+00 & 2.08E+00 & 56 & Second \\ \hline
151 & IOR & 2 & HDF5 Independent N-to-1  File Open Time (Read) & -18.2 & N & 7.01E-01 & 1.10E+00 & 22 & 5.74E-01 & 6.34E-01 & 56 & Second \\ \hline
152 & IOR & 2 & HDF5 Independent N-to-1  File Open Time (Write) & 4.1 & N & 2.24E-01 & 1.35E-01 & 22 & 2.33E-01 & 1.86E-01 & 56 & Second \\ \hline
153 & IOR & 2 & HDF5 Independent N-to-1 Read Aggregate Throughput & -1.9 & N & 1.95E+02 & 2.29E+01 & 22 & 1.92E+02 & 2.06E+01 & 56 & MByte per Second \\ \hline
154 & IOR & 2 & HDF5 Independent N-to-1 Write Aggregate Throughput & -3.6 & N & 1.59E+02 & 2.48E+01 & 22 & 1.54E+02 & 2.28E+01 & 56 & MByte per Second \\ \hline
155 & IOR & 2 & HDF5 N-to-N  File Close Time (Read) & 3.3 & N & 8.64E+00 & 1.04E+00 & 22 & 8.93E+00 & 9.28E-01 & 56 & Second \\ \hline
156 & IOR & 2 & HDF5 N-to-N  File Close Time (Write) & 1.4 & N & 1.41E+01 & 4.00E+00 & 22 & 1.43E+01 & 3.89E+00 & 56 & Second \\ \hline
157 & IOR & 2 & HDF5 N-to-N  File Open Time (Read) & 1.9 & N & 7.01E+00 & 8.88E-01 & 22 & 7.14E+00 & 1.01E+00 & 56 & Second \\ \hline
158 & IOR & 2 & HDF5 N-to-N  File Open Time (Write) & 5.1 & N & 8.34E+00 & 4.03E+00 & 22 & 8.77E+00 & 3.99E+00 & 56 & Second \\ \hline
159 & IOR & 2 & HDF5 N-to-N Read Aggregate Throughput & -0.2 & N & 2.45E+02 & 1.35E+01 & 22 & 2.44E+02 & 1.10E+01 & 56 & MByte per Second \\ \hline
160 & IOR & 2 & HDF5 N-to-N Write Aggregate Throughput & 1.2 & N & 2.07E+02 & 3.08E+01 & 22 & 2.10E+02 & 3.26E+01 & 56 & MByte per Second \\ \hline
161 & IOR & 2 & MPIIO Collective N-to-1  File Close Time (Read) & -18 & Y & 4.57E-02 & 1.49E-02 & 22 & 3.75E-02 & 7.93E-03 & 56 & Second \\ \hline
162 & IOR & 2 & MPIIO Collective N-to-1  File Close Time (Write) & -6.9 & N & 1.72E+00 & 5.64E-01 & 22 & 1.61E+00 & 4.25E-01 & 56 & Second \\ \hline
163 & IOR & 2 & MPIIO Collective N-to-1  File Open Time (Read) & 7.9 & N & 1.55E-01 & 3.98E-03 & 22 & 1.67E-01 & 7.67E-02 & 56 & Second \\ \hline
164 & IOR & 2 & MPIIO Collective N-to-1  File Open Time (Write) & 13.7 & N & 1.97E-01 & 1.20E-01 & 22 & 2.25E-01 & 1.71E-01 & 56 & Second \\ \hline
165 & IOR & 2 & MPIIO Collective N-to-1 Read Aggregate Throughput & 2.5 & N & 2.04E+02 & 1.34E+01 & 22 & 2.09E+02 & 2.11E+01 & 56 & MByte per Second \\ \hline
166 & IOR & 2 & MPIIO Collective N-to-1 Write Aggregate Throughput & -2.8 & N & 1.99E+02 & 3.66E+01 & 22 & 1.93E+02 & 2.59E+01 & 56 & MByte per Second \\ \hline
167 & IOR & 2 & MPIIO Independent N-to-1  File Close Time (Read) & 0.9 & N & 1.21E+01 & 1.45E+00 & 22 & 1.22E+01 & 1.44E+00 & 56 & Second \\ \hline
168 & IOR & 2 & MPIIO Independent N-to-1  File Close Time (Write) & 2.8 & N & 8.91E+00 & 3.37E+00 & 22 & 9.15E+00 & 3.14E+00 & 56 & Second \\ \hline
169 & IOR & 2 & MPIIO Independent N-to-1  File Open Time (Read) & 2.4 & Y & 1.51E-01 & 3.71E-03 & 22 & 1.55E-01 & 4.52E-03 & 56 & Second \\ \hline
170 & IOR & 2 & MPIIO Independent N-to-1  File Open Time (Write) & 7.5 & N & 2.40E-01 & 1.72E-01 & 22 & 2.58E-01 & 2.63E-01 & 56 & Second \\ \hline
171 & IOR & 2 & MPIIO Independent N-to-1 Read Aggregate Throughput & -1.2 & N & 2.04E+02 & 1.70E+01 & 22 & 2.01E+02 & 1.50E+01 & 56 & MByte per Second \\ \hline
172 & IOR & 2 & MPIIO Independent N-to-1 Write Aggregate Throughput & -3.7 & N & 1.62E+02 & 3.57E+01 & 22 & 1.56E+02 & 3.17E+01 & 56 & MByte per Second \\ \hline
173 & IOR & 2 & MPIIO N-to-N  File Close Time (Read) & 20.7 & Y & 5.76E+00 & 1.26E+00 & 22 & 6.95E+00 & 1.52E+00 & 56 & Second \\ \hline
174 & IOR & 2 & MPIIO N-to-N  File Close Time (Write) & -2.4 & N & 1.42E+01 & 3.66E+00 & 22 & 1.38E+01 & 2.46E+00 & 56 & Second \\ \hline
175 & IOR & 2 & MPIIO N-to-N  File Open Time (Read) & 58.9 & N & 1.17E+00 & 2.21E+00 & 22 & 1.86E+00 & 2.40E+00 & 56 & Second \\ \hline
176 & IOR & 2 & MPIIO N-to-N  File Open Time (Write) & -16.2 & N & 8.87E+00 & 2.99E+00 & 22 & 7.44E+00 & 3.40E+00 & 56 & Second \\ \hline
177 & IOR & 2 & MPIIO N-to-N Read Aggregate Throughput & -1.3 & N & 2.62E+02 & 7.73E+00 & 22 & 2.59E+02 & 8.82E+00 & 56 & MByte per Second \\ \hline
178 & IOR & 2 & MPIIO N-to-N Write Aggregate Throughput & 7.3 & N & 2.13E+02 & 3.83E+01 & 22 & 2.29E+02 & 2.99E+01 & 56 & MByte per Second \\ \hline
179 & IOR & 2 & Number of Tests Passed & 0 & N & 1.00E+01 & 0.00E+00 & 22 & 1.00E+01 & 0.00E+00 & 56 & NA \\ \hline
180 & IOR & 2 & Number of Tests Started & 0 & N & 2.00E+01 & 0.00E+00 & 22 & 2.00E+01 & 0.00E+00 & 56 & NA \\ \hline
181 & IOR & 2 & Parallel NetCDF Collective N-to-1  File Close Time (Read) & 6.3 & N & 5.43E-01 & 1.86E-01 & 22 & 5.77E-01 & 2.15E-01 & 56 & Second \\ \hline
182 & IOR & 2 & Parallel NetCDF Collective N-to-1  File Close Time (Write) & -2.5 & N & 4.51E-01 & 3.32E-01 & 22 & 4.40E-01 & 3.32E-01 & 56 & Second \\ \hline
183 & IOR & 2 & Parallel NetCDF Collective N-to-1  File Open Time (Read) & -1.5 & N & 2.25E-01 & 7.60E-02 & 22 & 2.22E-01 & 1.10E-01 & 56 & Second \\ \hline
184 & IOR & 2 & Parallel NetCDF Collective N-to-1  File Open Time (Write) & 46.4 & N & 1.77E-01 & 5.34E-02 & 22 & 2.58E-01 & 3.55E-01 & 56 & Second \\ \hline
185 & IOR & 2 & Parallel NetCDF Collective N-to-1 Read Aggregate Throughput & -1.6 & Y & 2.16E+02 & 3.49E+00 & 22 & 2.13E+02 & 1.11E+01 & 56 & MByte per Second \\ \hline
186 & IOR & 2 & Parallel NetCDF Collective N-to-1 Write Aggregate Throughput & 3 & N & 1.68E+02 & 1.92E+01 & 22 & 1.73E+02 & 2.54E+01 & 56 & MByte per Second \\ \hline
187 & IOR & 2 & Parallel NetCDF Independent N-to-1  File Close Time (Read) & 3.2 & N & 6.89E+00 & 2.37E+00 & 22 & 7.11E+00 & 2.49E+00 & 56 & Second \\ \hline
188 & IOR & 2 & Parallel NetCDF Independent N-to-1  File Close Time (Write) & 6.5 & N & 1.05E+01 & 3.74E+00 & 22 & 1.12E+01 & 5.12E+00 & 56 & Second \\ \hline
189 & IOR & 2 & Parallel NetCDF Independent N-to-1  File Open Time (Read) & 5.7 & N & 2.07E-01 & 5.17E-02 & 22 & 2.18E-01 & 8.09E-02 & 56 & Second \\ \hline
190 & IOR & 2 & Parallel NetCDF Independent N-to-1  File Open Time (Write) & 28.2 & Y & 1.65E-01 & 4.32E-03 & 22 & 2.12E-01 & 1.30E-01 & 56 & Second \\ \hline
191 & IOR & 2 & Parallel NetCDF Independent N-to-1 Read Aggregate Throughput & 0.2 & N & 2.08E+02 & 7.41E+00 & 22 & 2.08E+02 & 7.96E+00 & 56 & MByte per Second \\ \hline
192 & IOR & 2 & Parallel NetCDF Independent N-to-1 Write Aggregate Throughput & 1.8 & N & 1.51E+02 & 2.09E+01 & 22 & 1.54E+02 & 2.41E+01 & 56 & MByte per Second \\ \hline
193 & IOR & 2 & POSIX N-to-1  File Close Time (Read) & 3.9 & N & 1.17E+01 & 1.46E+00 & 22 & 1.21E+01 & 1.27E+00 & 56 & Second \\ \hline
194 & IOR & 2 & POSIX N-to-1  File Close Time (Write) & 5.2 & N & 2.56E+00 & 6.63E-01 & 22 & 2.69E+00 & 8.29E-01 & 56 & Second \\ \hline
195 & IOR & 2 & POSIX N-to-1  File Open Time (Read) & 0.5 & N & 5.36E-02 & 3.32E-03 & 22 & 5.39E-02 & 2.92E-03 & 56 & Second \\ \hline
196 & IOR & 2 & POSIX N-to-1  File Open Time (Write) & 86.5 & N & 8.50E-02 & 1.84E-01 & 22 & 1.59E-01 & 7.50E-01 & 56 & Second \\ \hline
197 & IOR & 2 & POSIX N-to-1 Read Aggregate Throughput & 0.4 & N & 2.02E+02 & 9.31E+00 & 22 & 2.03E+02 & 1.26E+01 & 56 & MByte per Second \\ \hline
198 & IOR & 2 & POSIX N-to-1 Write Aggregate Throughput & 0.1 & N & 2.33E+02 & 1.36E+01 & 22 & 2.33E+02 & 1.69E+01 & 56 & MByte per Second \\ \hline
199 & IOR & 2 & POSIX N-to-N  File Close Time (Read) & 4.8 & N & 5.39E+00 & 2.43E+00 & 22 & 5.64E+00 & 1.85E+00 & 56 & Second \\ \hline
200 & IOR & 2 & POSIX N-to-N  File Close Time (Write) & -5.3 & N & 1.18E+01 & 3.28E+00 & 22 & 1.12E+01 & 3.13E+00 & 56 & Second \\ \hline
201 & IOR & 2 & POSIX N-to-N  File Open Time (Read) & 26.6 & N & 3.06E+00 & 3.08E+00 & 22 & 3.88E+00 & 3.06E+00 & 56 & Second \\ \hline
202 & IOR & 2 & POSIX N-to-N  File Open Time (Write) & -20 & N & 8.43E+00 & 3.29E+00 & 22 & 6.75E+00 & 3.92E+00 & 56 & Second \\ \hline
203 & IOR & 2 & POSIX N-to-N Read Aggregate Throughput & 0.2 & N & 2.67E+02 & 3.25E+00 & 22 & 2.68E+02 & 2.43E+00 & 56 & MByte per Second \\ \hline
204 & IOR & 2 & POSIX N-to-N Write Aggregate Throughput & 3.2 & N & 2.29E+02 & 3.33E+01 & 22 & 2.36E+02 & 3.17E+01 & 56 & MByte per Second \\ \hline
205 & IOR & 2 & Wall Clock Time & 1.5 & N & 3.71E+02 & 1.22E+01 & 22 & 3.77E+02 & 1.95E+01 & 56 & Second \\ \hline
206 & IOR.local & 1 & HDF5 Collective N-to-1  File Close Time (Read) & 41.9 & Y & 1.16E-02 & 6.57E-03 & 12 & 1.65E-02 & 7.64E-03 & 56 & Second \\ \hline
207 & IOR.local & 1 & HDF5 Collective N-to-1  File Close Time (Write) & 81 & N & 1.02E-02 & 2.07E-03 & 12 & 1.85E-02 & 6.31E-02 & 56 & Second \\ \hline
208 & IOR.local & 1 & HDF5 Collective N-to-1  File Open Time (Read) & 3.8 & N & 5.78E-02 & 4.48E-03 & 12 & 6.01E-02 & 4.91E-03 & 56 & Second \\ \hline
209 & IOR.local & 1 & HDF5 Collective N-to-1  File Open Time (Write) & 14.6 & Y & 5.84E-02 & 4.36E-03 & 12 & 6.69E-02 & 8.12E-03 & 56 & Second \\ \hline
210 & IOR.local & 1 & HDF5 Collective N-to-1 Read Aggregate Throughput & -0.7 & N & 2.05E+02 & 3.59E+00 & 12 & 2.04E+02 & 1.80E+00 & 56 & MByte per Second \\ \hline
211 & IOR.local & 1 & HDF5 Collective N-to-1 Write Aggregate Throughput & -1.5 & N & 4.81E+01 & 3.84E+00 & 12 & 4.74E+01 & 4.11E+00 & 56 & MByte per Second \\ \hline
212 & IOR.local & 1 & HDF5 Independent N-to-1  File Close Time (Read) & -10.1 & Y & 4.28E-02 & 5.16E-03 & 12 & 3.85E-02 & 8.05E-03 & 56 & Second \\ \hline
213 & IOR.local & 1 & HDF5 Independent N-to-1  File Close Time (Write) & -0.5 & N & 3.31E+00 & 5.47E-01 & 12 & 3.29E+00 & 3.43E-01 & 56 & Second \\ \hline
214 & IOR.local & 1 & HDF5 Independent N-to-1  File Open Time (Read) & 7.6 & Y & 5.57E-02 & 3.66E-03 & 12 & 5.99E-02 & 4.41E-03 & 56 & Second \\ \hline
215 & IOR.local & 1 & HDF5 Independent N-to-1  File Open Time (Write) & 18.4 & Y & 5.60E-02 & 3.42E-03 & 12 & 6.63E-02 & 7.70E-03 & 56 & Second \\ \hline
216 & IOR.local & 1 & HDF5 Independent N-to-1 Read Aggregate Throughput & -1.1 & N & 2.61E+03 & 6.21E+01 & 12 & 2.58E+03 & 3.94E+01 & 56 & MByte per Second \\ \hline
217 & IOR.local & 1 & HDF5 Independent N-to-1 Write Aggregate Throughput & -2.4 & N & 2.90E+01 & 2.05E+00 & 12 & 2.84E+01 & 1.79E+00 & 56 & MByte per Second \\ \hline
218 & IOR.local & 1 & HDF5 N-to-N  File Close Time (Read) & 33.3 & N & 3.27E-02 & 5.93E-03 & 12 & 4.37E-02 & 6.77E-02 & 56 & Second \\ \hline
219 & IOR.local & 1 & HDF5 N-to-N  File Close Time (Write) & 14 & N & 6.84E-01 & 3.33E-01 & 12 & 7.80E-01 & 3.87E-01 & 56 & Second \\ \hline
220 & IOR.local & 1 & HDF5 N-to-N  File Open Time (Read) & 23.6 & N & 4.62E-02 & 3.40E-03 & 12 & 5.70E-02 & 5.32E-02 & 56 & Second \\ \hline
221 & IOR.local & 1 & HDF5 N-to-N  File Open Time (Write) & 22.6 & Y & 3.94E-02 & 1.58E-03 & 12 & 4.83E-02 & 1.35E-02 & 56 & Second \\ \hline
222 & IOR.local & 1 & HDF5 N-to-N Read Aggregate Throughput & -2.1 & Y & 2.47E+03 & 3.02E+01 & 12 & 2.42E+03 & 1.23E+02 & 56 & MByte per Second \\ \hline
223 & IOR.local & 1 & HDF5 N-to-N Write Aggregate Throughput & -1.4 & N & 3.58E+01 & 1.39E+00 & 12 & 3.53E+01 & 1.00E+00 & 56 & MByte per Second \\ \hline
224 & IOR.local & 1 & MPIIO Collective N-to-1  File Close Time (Read) & -9.7 & N & 3.50E-02 & 1.17E-02 & 12 & 3.16E-02 & 9.69E-03 & 56 & Second \\ \hline
225 & IOR.local & 1 & MPIIO Collective N-to-1  File Close Time (Write) & 0.7 & N & 3.80E+00 & 2.10E-01 & 12 & 3.83E+00 & 2.94E-01 & 56 & Second \\ \hline
226 & IOR.local & 1 & MPIIO Collective N-to-1  File Open Time (Read) & -1.1 & N & 5.54E-02 & 4.76E-03 & 12 & 5.48E-02 & 4.72E-03 & 56 & Second \\ \hline
227 & IOR.local & 1 & MPIIO Collective N-to-1  File Open Time (Write) & 13.6 & Y & 6.02E-02 & 2.81E-03 & 12 & 6.84E-02 & 2.49E-02 & 56 & Second \\ \hline
228 & IOR.local & 1 & MPIIO Collective N-to-1 Read Aggregate Throughput & -1.2 & Y & 2.50E+02 & 2.22E+00 & 12 & 2.47E+02 & 3.15E+00 & 56 & MByte per Second \\ \hline
229 & IOR.local & 1 & MPIIO Collective N-to-1 Write Aggregate Throughput & -0.8 & N & 3.73E+01 & 1.40E+00 & 12 & 3.70E+01 & 1.23E+00 & 56 & MByte per Second \\ \hline
230 & IOR.local & 1 & MPIIO Independent N-to-1  File Close Time (Read) & 10.5 & N & 3.59E-02 & 7.58E-03 & 12 & 3.97E-02 & 8.38E-03 & 56 & Second \\ \hline
231 & IOR.local & 1 & MPIIO Independent N-to-1  File Close Time (Write) & -1.3 & N & 3.73E+00 & 3.02E-01 & 12 & 3.68E+00 & 4.07E-01 & 56 & Second \\ \hline
232 & IOR.local & 1 & MPIIO Independent N-to-1  File Open Time (Read) & 0.4 & N & 5.58E-02 & 4.38E-03 & 12 & 5.61E-02 & 4.39E-03 & 56 & Second \\ \hline
233 & IOR.local & 1 & MPIIO Independent N-to-1  File Open Time (Write) & 10.7 & Y & 5.90E-02 & 3.85E-03 & 12 & 6.53E-02 & 2.20E-02 & 56 & Second \\ \hline
234 & IOR.local & 1 & MPIIO Independent N-to-1 Read Aggregate Throughput & -3.4 & Y & 2.67E+03 & 2.53E+01 & 12 & 2.58E+03 & 7.05E+01 & 56 & MByte per Second \\ \hline
235 & IOR.local & 1 & MPIIO Independent N-to-1 Write Aggregate Throughput & -14.1 & Y & 6.70E+01 & 7.77E+00 & 12 & 5.76E+01 & 1.07E+01 & 56 & MByte per Second \\ \hline
236 & IOR.local & 1 & MPIIO N-to-N  File Close Time (Read) & 32.1 & Y & 2.82E-02 & 6.01E-03 & 12 & 3.73E-02 & 8.04E-03 & 56 & Second \\ \hline
237 & IOR.local & 1 & MPIIO N-to-N  File Close Time (Write) & 0.7 & N & 7.07E-01 & 4.95E-01 & 12 & 7.12E-01 & 4.70E-01 & 56 & Second \\ \hline
238 & IOR.local & 1 & MPIIO N-to-N  File Open Time (Read) & 3.2 & N & 4.41E-02 & 3.65E-03 & 12 & 4.55E-02 & 4.03E-03 & 56 & Second \\ \hline
239 & IOR.local & 1 & MPIIO N-to-N  File Open Time (Write) & 10.7 & Y & 4.12E-02 & 4.03E-03 & 12 & 4.56E-02 & 6.33E-03 & 56 & Second \\ \hline
240 & IOR.local & 1 & MPIIO N-to-N Read Aggregate Throughput & -2.7 & Y & 2.72E+03 & 4.33E+01 & 12 & 2.65E+03 & 4.65E+01 & 56 & MByte per Second \\ \hline
241 & IOR.local & 1 & MPIIO N-to-N Write Aggregate Throughput & 1.7 & N & 3.71E+01 & 2.23E+00 & 12 & 3.78E+01 & 3.32E+00 & 56 & MByte per Second \\ \hline
242 & IOR.local & 1 & Number of Tests Passed & 0 & N & 1.00E+01 & 0.00E+00 & 12 & 1.00E+01 & 0.00E+00 & 56 & NA \\ \hline
243 & IOR.local & 1 & Number of Tests Started & 0 & N & 2.00E+01 & 0.00E+00 & 12 & 2.00E+01 & 0.00E+00 & 56 & NA \\ \hline
244 & IOR.local & 1 & Parallel NetCDF Collective N-to-1  File Close Time (Read) & 5.8 & N & 3.79E-03 & 1.23E-03 & 12 & 4.01E-03 & 1.05E-03 & 56 & Second \\ \hline
245 & IOR.local & 1 & Parallel NetCDF Collective N-to-1  File Close Time (Write) & -2 & N & 1.17E-02 & 9.13E-03 & 12 & 1.14E-02 & 7.57E-03 & 56 & Second \\ \hline
246 & IOR.local & 1 & Parallel NetCDF Collective N-to-1  File Open Time (Read) & 6.2 & Y & 6.44E-02 & 3.61E-03 & 12 & 6.84E-02 & 4.81E-03 & 56 & Second \\ \hline
247 & IOR.local & 1 & Parallel NetCDF Collective N-to-1  File Open Time (Write) & 63.3 & N & 6.12E-02 & 4.72E-03 & 12 & 9.99E-02 & 2.30E-01 & 56 & Second \\ \hline
248 & IOR.local & 1 & Parallel NetCDF Collective N-to-1 Read Aggregate Throughput & -1.9 & N & 2.57E+03 & 9.70E+01 & 12 & 2.53E+03 & 1.14E+02 & 56 & MByte per Second \\ \hline
249 & IOR.local & 1 & Parallel NetCDF Collective N-to-1 Write Aggregate Throughput & -3.8 & N & 8.01E+02 & 9.37E+01 & 12 & 7.70E+02 & 1.48E+02 & 56 & MByte per Second \\ \hline
250 & IOR.local & 1 & Parallel NetCDF Independent N-to-1  File Close Time (Read) & 9.6 & N & 6.65E-02 & 7.71E-03 & 12 & 7.28E-02 & 2.40E-02 & 56 & Second \\ \hline
251 & IOR.local & 1 & Parallel NetCDF Independent N-to-1  File Close Time (Write) & 8.7 & N & 5.75E+01 & 2.04E+01 & 12 & 6.25E+01 & 2.21E+01 & 56 & Second \\ \hline
252 & IOR.local & 1 & Parallel NetCDF Independent N-to-1  File Open Time (Read) & 9.3 & Y & 6.24E-02 & 3.43E-03 & 12 & 6.82E-02 & 4.62E-03 & 56 & Second \\ \hline
253 & IOR.local & 1 & Parallel NetCDF Independent N-to-1  File Open Time (Write) & 11.1 & Y & 6.05E-02 & 4.96E-03 & 12 & 6.72E-02 & 8.09E-03 & 56 & Second \\ \hline
254 & IOR.local & 1 & Parallel NetCDF Independent N-to-1 Read Aggregate Throughput & 4.4 & N & 5.70E+01 & 8.72E+00 & 12 & 5.95E+01 & 1.79E+01 & 56 & MByte per Second \\ \hline
255 & IOR.local & 1 & Parallel NetCDF Independent N-to-1 Write Aggregate Throughput & -4.8 & N & 1.49E+01 & 2.26E+00 & 12 & 1.42E+01 & 2.30E+00 & 56 & MByte per Second \\ \hline
256 & IOR.local & 1 & POSIX N-to-1  File Close Time (Read) & -68.1 & N & 9.90E-02 & 2.17E-01 & 12 & 3.16E-02 & 6.00E-03 & 56 & Second \\ \hline
257 & IOR.local & 1 & POSIX N-to-1  File Close Time (Write) & 1.6 & N & 1.93E-01 & 6.02E-02 & 12 & 1.96E-01 & 6.38E-02 & 56 & Second \\ \hline
258 & IOR.local & 1 & POSIX N-to-1  File Open Time (Read) & 3.2 & N & 4.77E-02 & 3.58E-03 & 12 & 4.93E-02 & 3.66E-03 & 56 & Second \\ \hline
259 & IOR.local & 1 & POSIX N-to-1  File Open Time (Write) & 5.9 & Y & 4.94E-02 & 2.77E-03 & 12 & 5.23E-02 & 5.16E-03 & 56 & Second \\ \hline
260 & IOR.local & 1 & POSIX N-to-1 Read Aggregate Throughput & 2.6 & N & 2.82E+03 & 4.90E+02 & 12 & 2.89E+03 & 6.28E+01 & 56 & MByte per Second \\ \hline
261 & IOR.local & 1 & POSIX N-to-1 Write Aggregate Throughput & -0.9 & N & 1.15E+03 & 5.33E+01 & 12 & 1.14E+03 & 4.99E+01 & 56 & MByte per Second \\ \hline
262 & IOR.local & 1 & POSIX N-to-N  File Close Time (Read) & 328.9 & Y & 3.22E-02 & 7.51E-03 & 12 & 1.38E-01 & 2.32E-01 & 56 & Second \\ \hline
263 & IOR.local & 1 & POSIX N-to-N  File Close Time (Write) & 84.7 & Y & 2.35E-02 & 7.99E-03 & 12 & 4.34E-02 & 2.70E-02 & 56 & Second \\ \hline
264 & IOR.local & 1 & POSIX N-to-N  File Open Time (Read) & -1.9 & N & 4.95E-02 & 5.36E-03 & 12 & 4.85E-02 & 3.67E-03 & 56 & Second \\ \hline
265 & IOR.local & 1 & POSIX N-to-N  File Open Time (Write) & 12.5 & Y & 4.86E-02 & 5.50E-03 & 12 & 5.47E-02 & 7.31E-03 & 56 & Second \\ \hline
266 & IOR.local & 1 & POSIX N-to-N Read Aggregate Throughput & -11.3 & Y & 2.73E+03 & 3.23E+01 & 12 & 2.42E+03 & 4.63E+02 & 56 & MByte per Second \\ \hline
267 & IOR.local & 1 & POSIX N-to-N Write Aggregate Throughput & -4.1 & Y & 9.13E+02 & 5.07E+01 & 12 & 8.76E+02 & 6.76E+01 & 56 & MByte per Second \\ \hline
268 & IOR.local & 1 & Wall Clock Time & 2.2 & N & 4.63E+02 & 1.64E+01 & 12 & 4.73E+02 & 1.90E+01 & 56 & Second \\ \hline
269 & MDTest & 1 & Directory creation (single directory per process) & -9.4 & Y & 1.01E+04 & 6.55E+02 & 21 & 9.13E+03 & 4.31E+02 & 56 & Operations/Second \\ \hline
270 & MDTest & 1 & Directory creation (single directory) & -11.2 & Y & 4.05E+03 & 1.35E+02 & 21 & 3.60E+03 & 1.87E+02 & 56 & Operations/Second \\ \hline
271 & MDTest & 1 & Directory creation (single tree directory per process) & -12.4 & Y & 6.00E+03 & 3.52E+02 & 21 & 5.26E+03 & 2.51E+02 & 56 & Operations/Second \\ \hline
272 & MDTest & 1 & Directory creation (single tree directory) & -15.1 & Y & 8.55E+03 & 3.26E+02 & 21 & 7.26E+03 & 3.91E+02 & 56 & Operations/Second \\ \hline
273 & MDTest & 1 & Directory removal (single directory per process) & -11.7 & Y & 2.31E+04 & 2.12E+03 & 21 & 2.04E+04 & 1.76E+03 & 56 & Operations/Second \\ \hline
274 & MDTest & 1 & Directory removal (single directory) & -17.7 & Y & 6.55E+03 & 2.45E+02 & 21 & 5.39E+03 & 2.65E+02 & 56 & Operations/Second \\ \hline
275 & MDTest & 1 & Directory removal (single tree directory per process) & -14.7 & Y & 2.15E+04 & 7.59E+02 & 21 & 1.83E+04 & 7.12E+02 & 56 & Operations/Second \\ \hline
276 & MDTest & 1 & Directory removal (single tree directory) & -16 & Y & 2.02E+04 & 7.18E+02 & 21 & 1.70E+04 & 7.99E+02 & 56 & Operations/Second \\ \hline
277 & MDTest & 1 & Directory stat (single directory per process) & -14.3 & N & 6.56E+05 & 2.20E+05 & 21 & 5.62E+05 & 1.56E+05 & 56 & Operations/Second \\ \hline
278 & MDTest & 1 & Directory stat (single directory) & -16.3 & N & 5.38E+05 & 2.01E+05 & 21 & 4.50E+05 & 1.38E+05 & 56 & Operations/Second \\ \hline
279 & MDTest & 1 & Directory stat (single tree directory per process) & -16.9 & Y & 1.69E+05 & 3.29E+04 & 21 & 1.40E+05 & 3.65E+04 & 56 & Operations/Second \\ \hline
280 & MDTest & 1 & Directory stat (single tree directory) & -18.4 & N & 1.90E+05 & 7.09E+04 & 21 & 1.55E+05 & 6.58E+04 & 56 & Operations/Second \\ \hline
281 & MDTest & 1 & File creation (single directory per process) & -5.2 & Y & 1.15E+04 & 9.73E+02 & 21 & 1.09E+04 & 8.95E+02 & 56 & Operations/Second \\ \hline
282 & MDTest & 1 & File creation (single directory) & -11.6 & Y & 3.65E+03 & 1.17E+02 & 21 & 3.23E+03 & 1.61E+02 & 56 & Operations/Second \\ \hline
283 & MDTest & 1 & File creation (single tree directory per process) & -13.6 & Y & 6.92E+03 & 3.64E+02 & 21 & 5.98E+03 & 3.67E+02 & 56 & Operations/Second \\ \hline
284 & MDTest & 1 & File creation (single tree directory) & -12.3 & Y & 8.09E+03 & 3.13E+02 & 21 & 7.10E+03 & 3.59E+02 & 56 & Operations/Second \\ \hline
285 & MDTest & 1 & File read (single directory per process) & -12.5 & Y & 6.31E+04 & 5.44E+03 & 21 & 5.52E+04 & 5.28E+03 & 56 & Operations/Second \\ \hline
286 & MDTest & 1 & File read (single directory) & -14.8 & Y & 4.89E+04 & 2.31E+03 & 21 & 4.17E+04 & 2.41E+03 & 56 & Operations/Second \\ \hline
287 & MDTest & 1 & File read (single tree directory per process) & -11.1 & Y & 3.19E+04 & 1.72E+03 & 21 & 2.83E+04 & 2.17E+03 & 56 & Operations/Second \\ \hline
288 & MDTest & 1 & File read (single tree directory) & -12.7 & Y & 3.28E+04 & 1.96E+03 & 21 & 2.86E+04 & 2.06E+03 & 56 & Operations/Second \\ \hline
289 & MDTest & 1 & File removal (single directory per process) & -12.6 & Y & 2.01E+04 & 1.30E+03 & 21 & 1.76E+04 & 1.16E+03 & 56 & Operations/Second \\ \hline
290 & MDTest & 1 & File removal (single directory) & -11 & Y & 3.05E+03 & 1.02E+02 & 21 & 2.72E+03 & 1.15E+02 & 56 & Operations/Second \\ \hline
291 & MDTest & 1 & File removal (single tree directory per process) & -12.4 & Y & 1.91E+04 & 9.95E+02 & 21 & 1.67E+04 & 9.62E+02 & 56 & Operations/Second \\ \hline
292 & MDTest & 1 & File removal (single tree directory) & -15.5 & Y & 1.33E+04 & 6.72E+02 & 21 & 1.13E+04 & 5.09E+02 & 56 & Operations/Second \\ \hline
293 & MDTest & 1 & File stat (single directory per process) & -11.3 & N & 6.59E+05 & 2.04E+05 & 21 & 5.85E+05 & 1.47E+05 & 56 & Operations/Second \\ \hline
294 & MDTest & 1 & File stat (single directory) & -14.6 & N & 5.33E+05 & 1.89E+05 & 21 & 4.55E+05 & 1.21E+05 & 56 & Operations/Second \\ \hline
295 & MDTest & 1 & File stat (single tree directory per process) & -20 & Y & 2.33E+05 & 8.27E+04 & 21 & 1.86E+05 & 5.37E+04 & 56 & Operations/Second \\ \hline
296 & MDTest & 1 & File stat (single tree directory) & -23.6 & Y & 2.16E+05 & 7.10E+04 & 21 & 1.65E+05 & 6.27E+04 & 56 & Operations/Second \\ \hline
297 & MDTest & 1 & Tree creation (single directory per process) & -10.4 & Y & 6.23E+02 & 8.82E+01 & 21 & 5.59E+02 & 7.81E+01 & 56 & Operations/Second \\ \hline
298 & MDTest & 1 & Tree creation (single directory) & -11 & Y & 4.53E+03 & 3.84E+02 & 21 & 4.03E+03 & 2.50E+02 & 56 & Operations/Second \\ \hline
299 & MDTest & 1 & Tree creation (single tree directory per process) & -11.4 & Y & 1.39E+03 & 5.54E+01 & 21 & 1.24E+03 & 5.32E+01 & 56 & Operations/Second \\ \hline
300 & MDTest & 1 & Tree creation (single tree directory) & -18.5 & Y & 7.00E+03 & 2.59E+02 & 21 & 5.71E+03 & 3.36E+02 & 56 & Operations/Second \\ \hline
301 & MDTest & 1 & Tree removal (single directory per process) & -7.6 & Y & 6.84E+02 & 5.68E+01 & 21 & 6.32E+02 & 5.64E+01 & 56 & Operations/Second \\ \hline
302 & MDTest & 1 & Tree removal (single directory) & -12.6 & Y & 2.68E+03 & 1.46E+02 & 21 & 2.34E+03 & 1.69E+02 & 56 & Operations/Second \\ \hline
303 & MDTest & 1 & Tree removal (single tree directory per process) & -17.1 & Y & 3.03E+03 & 1.39E+02 & 21 & 2.51E+03 & 1.45E+02 & 56 & Operations/Second \\ \hline
304 & MDTest & 1 & Tree removal (single tree directory) & -20.4 & Y & 7.28E+03 & 2.24E+02 & 21 & 5.80E+03 & 2.65E+02 & 56 & Operations/Second \\ \hline
305 & MDTest & 1 & Wall Clock Time & 24.1 & Y & 3.05E+01 & 3.17E+00 & 21 & 3.78E+01 & 4.10E+00 & 56 & Second \\ \hline
306 & MDTest & 2 & Directory creation (single directory per process) & -14.1 & Y & 1.76E+04 & 9.03E+02 & 23 & 1.51E+04 & 1.62E+03 & 55 & Operations/Second \\ \hline
307 & MDTest & 2 & Directory creation (single directory) & -6.2 & Y & 2.06E+02 & 2.12E+01 & 23 & 1.93E+02 & 1.44E+01 & 55 & Operations/Second \\ \hline
308 & MDTest & 2 & Directory creation (single tree directory per process) & -14.7 & Y & 1.13E+04 & 8.30E+02 & 23 & 9.63E+03 & 6.71E+02 & 55 & Operations/Second \\ \hline
309 & MDTest & 2 & Directory creation (single tree directory) & -9.8 & Y & 4.30E+03 & 2.38E+02 & 23 & 3.88E+03 & 3.44E+02 & 55 & Operations/Second \\ \hline
310 & MDTest & 2 & Directory removal (single directory per process) & -19.3 & Y & 4.49E+04 & 2.05E+03 & 23 & 3.62E+04 & 5.45E+03 & 55 & Operations/Second \\ \hline
311 & MDTest & 2 & Directory removal (single directory) & -6.5 & Y & 1.66E+02 & 6.87E+00 & 23 & 1.55E+02 & 7.43E+00 & 55 & Operations/Second \\ \hline
312 & MDTest & 2 & Directory removal (single tree directory per process) & -18 & Y & 3.90E+04 & 2.30E+03 & 23 & 3.20E+04 & 3.28E+03 & 55 & Operations/Second \\ \hline
313 & MDTest & 2 & Directory removal (single tree directory) & -8.5 & Y & 3.27E+03 & 2.92E+02 & 23 & 2.99E+03 & 2.68E+02 & 55 & Operations/Second \\ \hline
314 & MDTest & 2 & Directory stat (single directory per process) & -11.3 & N & 1.13E+06 & 5.01E+05 & 23 & 9.98E+05 & 3.50E+05 & 55 & Operations/Second \\ \hline
315 & MDTest & 2 & Directory stat (single directory) & -14.8 & N & 9.98E+04 & 5.19E+04 & 23 & 8.51E+04 & 6.43E+04 & 55 & Operations/Second \\ \hline
316 & MDTest & 2 & Directory stat (single tree directory per process) & -12.3 & Y & 2.52E+05 & 6.14E+04 & 23 & 2.21E+05 & 5.74E+04 & 55 & Operations/Second \\ \hline
317 & MDTest & 2 & Directory stat (single tree directory) & -10.3 & Y & 2.81E+04 & 1.86E+03 & 23 & 2.53E+04 & 2.25E+03 & 55 & Operations/Second \\ \hline
318 & MDTest & 2 & File creation (single directory per process) & -13.9 & Y & 2.46E+04 & 1.24E+03 & 23 & 2.12E+04 & 2.38E+03 & 55 & Operations/Second \\ \hline
319 & MDTest & 2 & File creation (single directory) & -5 & Y & 1.48E+02 & 4.61E+00 & 23 & 1.40E+02 & 4.80E+00 & 55 & Operations/Second \\ \hline
320 & MDTest & 2 & File creation (single tree directory per process) & -15.7 & Y & 1.32E+04 & 8.87E+02 & 23 & 1.11E+04 & 9.55E+02 & 55 & Operations/Second \\ \hline
321 & MDTest & 2 & File creation (single tree directory) & -7.3 & Y & 2.25E+03 & 1.08E+02 & 23 & 2.09E+03 & 1.67E+02 & 55 & Operations/Second \\ \hline
322 & MDTest & 2 & File read (single directory per process) & -14.3 & Y & 1.09E+05 & 1.19E+04 & 23 & 9.36E+04 & 1.42E+04 & 55 & Operations/Second \\ \hline
323 & MDTest & 2 & File read (single directory) & -26.8 & Y & 8.37E+04 & 9.20E+03 & 23 & 6.13E+04 & 9.08E+03 & 55 & Operations/Second \\ \hline
324 & MDTest & 2 & File read (single tree directory per process) & -14.7 & Y & 6.12E+04 & 5.28E+03 & 23 & 5.22E+04 & 6.70E+03 & 55 & Operations/Second \\ \hline
325 & MDTest & 2 & File read (single tree directory) & -24.4 & Y & 5.94E+04 & 2.90E+03 & 23 & 4.50E+04 & 4.92E+03 & 55 & Operations/Second \\ \hline
326 & MDTest & 2 & File removal (single directory per process) & -15.4 & Y & 3.93E+04 & 2.16E+03 & 23 & 3.32E+04 & 3.14E+03 & 55 & Operations/Second \\ \hline
327 & MDTest & 2 & File removal (single directory) & -4.8 & Y & 2.06E+02 & 7.66E+00 & 23 & 1.96E+02 & 6.98E+00 & 55 & Operations/Second \\ \hline
328 & MDTest & 2 & File removal (single tree directory per process) & -14.6 & Y & 3.60E+04 & 2.62E+03 & 23 & 3.08E+04 & 3.50E+03 & 55 & Operations/Second \\ \hline
329 & MDTest & 2 & File removal (single tree directory) & -10.5 & Y & 1.62E+03 & 1.25E+02 & 23 & 1.45E+03 & 9.63E+01 & 55 & Operations/Second \\ \hline
330 & MDTest & 2 & File stat (single directory per process) & -9.4 & N & 1.17E+06 & 5.10E+05 & 23 & 1.06E+06 & 3.24E+05 & 55 & Operations/Second \\ \hline
331 & MDTest & 2 & File stat (single directory) & 17.7 & N & 7.55E+05 & 4.30E+05 & 23 & 8.89E+05 & 3.30E+05 & 55 & Operations/Second \\ \hline
332 & MDTest & 2 & File stat (single tree directory per process) & -14.5 & Y & 3.00E+05 & 8.38E+04 & 23 & 2.56E+05 & 6.94E+04 & 55 & Operations/Second \\ \hline
333 & MDTest & 2 & File stat (single tree directory) & -10 & Y & 2.19E+04 & 1.62E+03 & 23 & 1.97E+04 & 1.28E+03 & 55 & Operations/Second \\ \hline
334 & MDTest & 2 & Tree creation (single directory per process) & -9.8 & Y & 7.09E+01 & 4.54E+00 & 23 & 6.40E+01 & 6.69E+00 & 55 & Operations/Second \\ \hline
335 & MDTest & 2 & Tree creation (single directory) & -15.3 & Y & 5.18E+03 & 5.15E+02 & 23 & 4.39E+03 & 4.04E+02 & 55 & Operations/Second \\ \hline
336 & MDTest & 2 & Tree creation (single tree directory per process) & -10.8 & Y & 5.32E+02 & 3.35E+01 & 23 & 4.75E+02 & 3.63E+01 & 55 & Operations/Second \\ \hline
337 & MDTest & 2 & Tree creation (single tree directory) & -14.6 & Y & 6.35E+03 & 3.06E+02 & 23 & 5.42E+03 & 5.64E+02 & 55 & Operations/Second \\ \hline
338 & MDTest & 2 & Tree removal (single directory per process) & -6.6 & Y & 1.75E+01 & 8.76E-01 & 23 & 1.63E+01 & 7.86E-01 & 55 & Operations/Second \\ \hline
339 & MDTest & 2 & Tree removal (single directory) & -10.3 & Y & 2.61E+02 & 4.03E+01 & 23 & 2.34E+02 & 3.26E+01 & 55 & Operations/Second \\ \hline
340 & MDTest & 2 & Tree removal (single tree directory per process) & -12.2 & Y & 5.98E+02 & 5.45E+01 & 23 & 5.25E+02 & 5.20E+01 & 55 & Operations/Second \\ \hline
341 & MDTest & 2 & Tree removal (single tree directory) & -4.5 & N & 9.29E+02 & 2.25E+02 & 23 & 8.88E+02 & 2.19E+02 & 55 & Operations/Second \\ \hline
342 & MDTest & 2 & Wall Clock Time & 9.7 & Y & 1.67E+02 & 3.60E+00 & 23 & 1.83E+02 & 5.30E+00 & 55 & Second \\ \hline
343 & MDTest.local & 1 & Directory creation (single directory per process) & 5.5 & Y & 1.04E+05 & 1.79E+03 & 12 & 1.10E+05 & 6.10E+03 & 56 & Operations/Second \\ \hline
344 & MDTest.local & 1 & Directory creation (single directory) & -6.6 & Y & 3.84E+04 & 3.12E+03 & 12 & 3.59E+04 & 3.59E+03 & 56 & Operations/Second \\ \hline
345 & MDTest.local & 1 & Directory creation (single tree directory per process) & 14.9 & Y & 1.10E+05 & 8.27E+03 & 12 & 1.27E+05 & 9.70E+03 & 56 & Operations/Second \\ \hline
346 & MDTest.local & 1 & Directory creation (single tree directory) & 2 & N & 1.04E+05 & 7.44E+03 & 12 & 1.06E+05 & 8.49E+03 & 56 & Operations/Second \\ \hline
347 & MDTest.local & 1 & Directory removal (single directory per process) & 7.9 & Y & 1.08E+05 & 6.99E+03 & 12 & 1.17E+05 & 9.71E+03 & 56 & Operations/Second \\ \hline
348 & MDTest.local & 1 & Directory removal (single directory) & -12.6 & Y & 4.92E+04 & 1.72E+03 & 12 & 4.30E+04 & 4.86E+03 & 56 & Operations/Second \\ \hline
349 & MDTest.local & 1 & Directory removal (single tree directory per process) & -0.2 & N & 1.40E+05 & 5.19E+03 & 12 & 1.40E+05 & 6.19E+03 & 56 & Operations/Second \\ \hline
350 & MDTest.local & 1 & Directory removal (single tree directory) & -11.1 & Y & 1.30E+05 & 3.70E+03 & 12 & 1.15E+05 & 1.08E+04 & 56 & Operations/Second \\ \hline
351 & MDTest.local & 1 & Directory stat (single directory per process) & -30.6 & Y & 1.77E+06 & 1.23E+05 & 12 & 1.23E+06 & 1.36E+05 & 56 & Operations/Second \\ \hline
352 & MDTest.local & 1 & Directory stat (single directory) & -29.9 & Y & 1.89E+06 & 1.77E+05 & 12 & 1.33E+06 & 1.38E+05 & 56 & Operations/Second \\ \hline
353 & MDTest.local & 1 & Directory stat (single tree directory per process) & -26.4 & Y & 1.88E+06 & 4.65E+04 & 12 & 1.39E+06 & 4.79E+04 & 56 & Operations/Second \\ \hline
354 & MDTest.local & 1 & Directory stat (single tree directory) & -25.6 & Y & 1.92E+06 & 5.72E+04 & 12 & 1.43E+06 & 4.68E+04 & 56 & Operations/Second \\ \hline
355 & MDTest.local & 1 & File creation (single directory per process) & -27.7 & Y & 2.41E+05 & 9.40E+04 & 12 & 1.74E+05 & 1.34E+04 & 56 & Operations/Second \\ \hline
356 & MDTest.local & 1 & File creation (single directory) & 0 & N & 7.38E+04 & 1.88E+03 & 12 & 7.38E+04 & 2.02E+04 & 56 & Operations/Second \\ \hline
357 & MDTest.local & 1 & File creation (single tree directory per process) & -2.3 & N & 2.03E+05 & 1.79E+04 & 12 & 1.98E+05 & 1.39E+04 & 56 & Operations/Second \\ \hline
358 & MDTest.local & 1 & File creation (single tree directory) & -10.9 & Y & 1.79E+05 & 1.45E+04 & 12 & 1.59E+05 & 1.54E+04 & 56 & Operations/Second \\ \hline
359 & MDTest.local & 1 & File read (single directory per process) & -31.9 & Y & 1.40E+06 & 1.61E+05 & 12 & 9.55E+05 & 1.05E+05 & 56 & Operations/Second \\ \hline
360 & MDTest.local & 1 & File read (single directory) & -27.4 & Y & 1.38E+06 & 9.98E+04 & 12 & 1.00E+06 & 1.00E+05 & 56 & Operations/Second \\ \hline
361 & MDTest.local & 1 & File read (single tree directory per process) & -24.7 & Y & 1.38E+06 & 2.22E+04 & 12 & 1.04E+06 & 2.38E+04 & 56 & Operations/Second \\ \hline
362 & MDTest.local & 1 & File read (single tree directory) & -25.1 & Y & 1.39E+06 & 3.10E+04 & 12 & 1.04E+06 & 2.62E+04 & 56 & Operations/Second \\ \hline
363 & MDTest.local & 1 & File removal (single directory per process) & -7.7 & Y & 2.00E+05 & 1.16E+04 & 12 & 1.85E+05 & 1.68E+04 & 56 & Operations/Second \\ \hline
364 & MDTest.local & 1 & File removal (single directory) & -5.5 & Y & 1.32E+05 & 5.42E+03 & 12 & 1.25E+05 & 1.67E+04 & 56 & Operations/Second \\ \hline
365 & MDTest.local & 1 & File removal (single tree directory per process) & -7.9 & Y & 2.10E+05 & 3.76E+03 & 12 & 1.93E+05 & 1.08E+04 & 56 & Operations/Second \\ \hline
366 & MDTest.local & 1 & File removal (single tree directory) & -8.6 & Y & 2.08E+05 & 7.99E+03 & 12 & 1.90E+05 & 1.53E+04 & 56 & Operations/Second \\ \hline
367 & MDTest.local & 1 & File stat (single directory per process) & -31.2 & Y & 1.78E+06 & 1.36E+05 & 12 & 1.23E+06 & 1.11E+05 & 56 & Operations/Second \\ \hline
368 & MDTest.local & 1 & File stat (single directory) & -30.2 & Y & 1.89E+06 & 1.94E+05 & 12 & 1.32E+06 & 1.50E+05 & 56 & Operations/Second \\ \hline
369 & MDTest.local & 1 & File stat (single tree directory per process) & -26.2 & Y & 1.91E+06 & 4.96E+04 & 12 & 1.41E+06 & 3.28E+04 & 56 & Operations/Second \\ \hline
370 & MDTest.local & 1 & File stat (single tree directory) & -26.3 & Y & 1.92E+06 & 5.17E+04 & 12 & 1.41E+06 & 2.97E+04 & 56 & Operations/Second \\ \hline
371 & MDTest.local & 1 & Tree creation (single directory per process) & -7.7 & Y & 3.28E+03 & 3.05E+02 & 12 & 3.03E+03 & 2.44E+02 & 56 & Operations/Second \\ \hline
372 & MDTest.local & 1 & Tree creation (single directory) & -3.7 & N & 2.10E+04 & 5.82E+03 & 12 & 2.02E+04 & 5.90E+03 & 56 & Operations/Second \\ \hline
373 & MDTest.local & 1 & Tree creation (single tree directory per process) & -2.9 & N & 9.69E+03 & 5.86E+02 & 12 & 9.41E+03 & 8.28E+02 & 56 & Operations/Second \\ \hline
374 & MDTest.local & 1 & Tree creation (single tree directory) & 5.9 & N & 3.32E+04 & 3.99E+03 & 12 & 3.52E+04 & 3.36E+03 & 56 & Operations/Second \\ \hline
375 & MDTest.local & 1 & Tree removal (single directory per process) & -5.2 & Y & 2.87E+03 & 9.87E+01 & 12 & 2.72E+03 & 2.51E+02 & 56 & Operations/Second \\ \hline
376 & MDTest.local & 1 & Tree removal (single directory) & -14.3 & Y & 5.73E+03 & 9.60E+02 & 12 & 4.91E+03 & 1.20E+03 & 56 & Operations/Second \\ \hline
377 & MDTest.local & 1 & Tree removal (single tree directory per process) & -8.4 & Y & 1.43E+04 & 8.18E+02 & 12 & 1.31E+04 & 1.34E+03 & 56 & Operations/Second \\ \hline
378 & MDTest.local & 1 & Tree removal (single tree directory) & -12.7 & Y & 2.32E+04 & 7.89E+02 & 12 & 2.03E+04 & 2.15E+03 & 56 & Operations/Second \\ \hline
379 & MDTest.local & 1 & Wall Clock Time & 78.6 & Y & 3.75E+00 & 6.22E-01 & 12 & 6.70E+00 & 2.61E+00 & 56 & Second \\ \hline
\end{tabular}
\end{table*}
